A Scalable Framework For Real-Time Multi-Robot, Multi-Human Collision Avoidance

Robust motion planning is a well-studied problem in the robotics literature, yet current algorithms struggle to operate scalably and safely in the presence of other moving agents, such as humans. This paper introduces a novel framework for robot navigation that accounts for high-order system dynamics and maintains safety in the presence of external disturbances, other robots, and non-deterministic intentional agents. Our approach precomputes a tracking error margin for each robot, generates confidence-aware human motion predictions, and coordinates multiple robots with a sequential priority ordering, effectively enabling scalable safe trajectory planning and execution. We demonstrate our approach in hardware with two robots and two humans. We also showcase our work's scalability in a larger simulation.

==> problem.tex <==
\section{problem statement}
\label{sec:problem}
We consider multiple communicative robots moving to individual goal locations in a shared space with multiple %non-communicative agents, including robots and 
humans. We assume that the robots can share future trajectories with each other, but that human %and non-communicative robot 
motion must be anticipated. \shnote{assumptions on human motion}. The robots should maintain a safe distance from each other and the humans at all times while working toward their respective goals.T his theory is presented in a general format, but for illustration purposes we use a running example of three quadcopters navigating around two humans.

\subsection{Robot Motion Model}
\label{subsec:robot_motion_model}
\shnote{copied from STP paper}
Consider $N$ robots $\R_i,i=1\ldots,N$, each trying to reach one of $N$ goal sets $\target_i,i=1\ldots,N$, while avoiding obstacles and collision with each other. Each robot $i$ has states $\x_{R,i}\in \R^{n_i}$ and moves with the following dynamics:

\begin{equation} \label{eq:dyn}
\dotx_{R,i} = f_{R,i} (\x_{R,i}, \ctrl_{R,i}), %\quad\x_{R,i}(\ti_{R,i}) = \x_{R,i}^0 
\end{equation}

\noindent where $\x_{R,i}$ is robot $i$'s state %with initial condition $\x_i^0$, 
and $\ctrl_i \in \mathbb{R}^{m_{R,i}}$ represents the robot's control actions. The dynamics $f_{R,i}(\cdot,\cdot)$ of the robot are individual and can be different across the team of robots.
Each robot $\R_i$ must avoid collision with respect to every other robot $\R_j, j\neq i$.  We define pairwise robot keep-out sets $\danger_{R_i,R_j} \subset \mathbb{R}^{n_{R_i}} \times \mathbb{R}^{n_{R_j}}$, which are the set of joint robot-robot states to be avoided due to collisions.

Given $M$ pedestrians, humans $H_i, i=1\ldots,M$ are similarly modeled with the following dynamics:
\begin{equation} \label{eq:dyn}
\dotx_{H,i} = f_{H,i} (\x_{H,i}, \ctrl_{H,i}), %\quad\x_{R,i}(\ti_{R,i}) = \x_{R,i}^0 
\end{equation}

For each robot we define a human keep-out set as $\danger_{R_i,H}$ as the set of joint states between the robot and all humans that are to be avoided, e.g. because they imply physical collisions between the robot and at least one human. Therefore, each robot must stay safe with respect to every preceding robot ($\danger_{R_i,R_j}$) and all humans ($\danger_{R_i,H}$).


%In general, the above problem must be analyzed in the joint state space of all vehicles, making the solution intractable. In this paper, we will instead consider the problem of performing path planning of the vehicles in a sequential manner. Without loss of generality, we consider the problem of first fixing $i=1$ and determining the optimal control for vehicle $1$, the vehicle with the highest priority. The resulting optimal control $\ctrl_1$ sends vehicle $1$ to $\target_1$ in minimum time. 

%Then, we plan the minimum time trajectory for each of the vehicles $2,\ldots,N$, in decreasing order of priority, given the previously-determined trajectories for higher-priority vehicles $1,\ldots,i-1$. We assume that all vehicles have complete information about the states and trajectories of higher-priority vehicles, and that all vehicles adhere to their planned trajectories. Thus, in planning its trajectory, vehicle $i$ treats higher-priority vehicles as known time-varying obstacles. 

%With the above sequential path planning (SPP) protocol and assumptions, our problem now reduces to the following for vehicle $i$. Given $\x_j(\cdot), j=1,\ldots,i-1$, determine $\ctrl_i(\cdot)$ that maximizes $\ti_i$ and such that $x_i(\tau) \in \target_i, \tau\le \tf_i$.


\subsection{Human Predictive Model}
\begin{itemize}
    \item copy/paste from RSS paper
    \item talk about how this changes for multiple humans
\end{itemize}
% We consider a single robot moving to a preset goal location in a space shared with a single human, and assume that the human expects the robot to avoid her.
% Therefore, it is the robot's responsibility to maintain a safe distance from the human at all times.
% We present our theory for a general single human and single robot setting, and use the running example of quadcopter navigating around a walking human to illustrate the proposed approach and demonstrate the utility of our method.

% \subsection{Motion Model}
% \label{subsec:robot_motion_model}

% Let the state of the human be $x_H \in \mathbb{R}^{n_H}$, where $n_H$ is the dimension of the human state space. 
% We similarly define the robot's state, for planning purposes, as  $x_R \in \mathbb{R}^{n_R}$.
% These states could represent the positions and velocities of a mobile robot and a human in a shared environment or the kinematic configurations of a human and a robotic manipulator in a common workspace.
% The human and robot are each modeled by their dynamics:
% \begin{equation}
%     \begin{aligned}
%     \dot{x}_H &= f_H(x_H, u_H) \qquad
%     \dot{x}_R &= f_R(x_R, u_R)
%     \end{aligned}
% \end{equation}
% where $u_H \in \mathbb{R}^{m_H}$ and $u_R \in \mathbb{R}^{m_R}$ are the control actions of the human and robot, respectively.

% The robot ultimately needs to plan and execute a trajectory to a goal state
% according to some notion of efficiency,
% while avoiding collisions with the human. %\adnote{we also care about efficiency}
% We define the keep-out set $\mathcal{K} \subset \mathbb{R}^{n_H} \times \mathbb{R}^{n_R}$ as the set of joint robot-human states to be avoided, e.g. because they imply physical collisions.
% To avoid reaching this set, the robot must reason about the human's future motion when constructing its own motion plan.

% \example{
% We introduce a running example for illustration throughout the paper.
% In this example we consider a small quadcopter that needs to fly to locations $g_R \in \mathbb{R}^3$ in a room where a human is walking.
% For the purposes of planning, the quadcopter's 3D state is given by its position in space $x_R = [p_x, p_y, p_z]$, with velocity controls assumed decoupled in each spatial direction, up to $v_R=0.25$~m/s.
% The human can only move by walking and therefore her state is given by planar coordinates $x_H = [h_x, h_y]$ evolving as $\dot{x}_H = [v_H \cos\phi_H, v_H \sin\phi_H]$.
% At any given time, the human is assumed to either move at a leisurely walking speed (${v_H \approx 1}$~m/s) or remain still (${v_H \approx 0}$).
% \\ \indent
% In this example, $\mathcal{K}$ consists of joint robot-human states in which the quadcopter is flying within a square of side length $l=0.3$~m centered around the human's location, while at
% any altitude, as well as any joint states in which the robot is outside the bounds of a box with a square base of side $L=3.66$~m and height $H=2$~m, regardless of the human's state.}

% \subsection{Robot Dynamics}

% Ideally, robots should plan their motion based on a high-fidelity model of their dynamics, accounting for inertia, actuator limits, and environment disturbances.
% Unfortunately, reasoning with such complex models is almost always computationally prohibitive.% \todo{is almost always too much?}
%  As a result, the models used for planning typically constitute a simplified representation of the physical dynamics of the real robot, and are therefore subject to some error that can have critical implications for safety. In particular, let $s_R\in\mathbb{R}^{n_S}$ denote the state of the robot in the higher-fidelity dynamical model, and let ${\pi:\mathbb{R}^{n_S}\to\mathbb{R}^{n_R}}$ be a known function that projects this higher-fidelity state onto a corresponding planning state, i.e $x_R = \pi(s_R)$. A planner which operates on $x_R$ may generate a trajectory which is difficult to track or even infeasible under the more accurate dynamical model.
% Thus reasoning with the planning model alone is not sufficient to guarantee safety for the real robot.


% \example{
%     We model our quadcopter with the following flight dynamics (in near-hover regime):\\
%     \noindent
%     \begin{equation}
%         \small \label{eq:Quad6D_dyn}
%         \begin{bmatrix}
%             \dot p_{x}\\ \dot p_{y}\\ \dot p_{z}
%         \end{bmatrix}
%         = \begin{bmatrix}
%             v_{x} \\ v_{y} \\ v_{z} \
%         \end{bmatrix}
%         \enspace ,\begin{bmatrix}
%              \dot v_{x}\\ \dot v_{y}\\ \dot v_{z}\\
%         \end{bmatrix}
%         = \begin{bmatrix}
%               g \tan\theta\\ -g \tan\phi \\ \tau - g 
%         \end{bmatrix}
%         \enspace,
%     \end{equation}
%     where $[p_x,p_y,p_z]$ is the quadcopter's position in space and $[v_x,v_y,v_z]$ is its velocity expressed in the fixed world frame, with thrust $\tau$ and attitude angles (roll $\phi$ and pitch $\theta$) as controls.
%     %\\ \indent
%     The quadcopter's motion planner generates nominal kinematic trajectories in the lower-dimensional $[p_x,p_y,p_z]$ position state space.
%     Therefore we have a linear projection map ${\pi(s_R) = [I_3, 0_3] s_R}$, that is, $x_R$ retains the position variables in $s_R$ and discards the velocities.
% }

% \subsection{Predictive Human Model}

% The robot has a predictive model of the human's motion, based on a set of parameters whose values may be inferred under a Bayesian framework or otherwise estimated over time.
% Extensive work in econometrics and cognitive science has shown that human behavior can be well modeled by utility-driven optimization \cite{von1945theory, luce1959individual, baker2007goal}.
% Thus, the robot models the human as optimizing a reward function, $r_H(x_H,u_H; \theta)$, that depends on the human's state and action, as well as a set of parameters $\theta$. This reward function could be a linear combination of features as in many inverse optimal control implementations (where the weighting $\theta$ between the features needs to be learned), or more generally learned through function approximators such as deep neural networks (where~$\theta$ are the trained weights) \cite{finn2016guided}.

% We assume that the robot has a suitable human reward function, either learned offline from prior human demonstrations or otherwise encoded by the system designers. 
% With this, the robot can compute the human's policy as a probability distribution over actions conditioned on the state.
% Using maximum-entropy assumptions \cite{ziebart2008maximum} and inspiration from noisy-rationality models used in cognitive science \cite{baker2007goal}, the robot models the human as more likely to choose actions with high expected utility, in this case the state-action value (or Q-value):
%   \begin{equation}
%     \label{eq:observation_model}
%         P(u^t_H \mid x^t_H; \beta, \theta) = \frac{e^{\beta Q_H(x^t_H,u^t_H; \theta)}}{\sum_{\tilde u}e^{\beta Q_H(x^t_H,\tilde u; \theta)}}\enspace.
%     \end{equation}

% \example{
%     The quadcopter's model of the human assumes that she intends to reach some target location $g\in\mathbb{R}^2$ in the most direct way possible. The human's reward function is given by the distance traveled $ 
%         \label{eq:reward}
%         r_H(x_H,u_H;g) = - ||u_H||_2 \enspace$
%     and human trajectories are constrained to terminate at $g$.
%     The state-action value, parametrized by ${\theta=g}$, captures the optimal cost of reaching $g$ from $x_H$ when initially applying $u_H$:
%     $
%         \label{eq:value}
%         Q_H(x_H,u_H;g) = -||u_H||_2 - ||x_H+u_H-g||_2 .
%     $
%     }

% The coefficient $\beta$ is traditionally called the \textit{rationality coefficient} and it determines the degree to which the robot expects to observe human actions aligned with its model of utility. 
  
% A common interpretation of $\beta = 0$ is a human who appears ``irrational," choosing actions uniformly at random and completely ignoring the modeled utility,    while $\beta \rightarrow \infty$ corresponds a ``perfectly rational" human.

% Instead, we believe that $\beta$ can be given a more pragmatic interpretation related to the accuracy with which the robot's model of the human is able to explain her motion.
% Consistently, in this paper, we refer to $\beta$ as \textit{model confidence}.

% Note that we assume the human does not react to the robot. This assumption can realistically capture plausible shared-space settings in which lightweight robots (e.g. micro-drones) may be expected to carry out services such as indoor surveillance in a building while minimizing interference with human activity.
% Additionally, to the extent that a more compliant human will tend to avoid collisions with the robot, the robot may still benefit in such scenarios---it is merely not assuming any cooperation \textit{a priori} in its planning.

% \subsection{Probabilistic Safe Motion Planning Problem}
% \label{subsec:prob_safe_motion_planning}

% The problem that the robot needs to solve is to plan a trajectory that, when tracked by the physical system, will reach a goal state as efficiently as possible while avoiding collisions with high confidence, based on an informed prediction of the human's future motion.

% Since any theoretical guarantee is tied to the model it is based on, 
% safety guarantees will inherit the probabilistic nature of human predictions.
% This induces a fundamental tradeoff between safety and \textit{liveness}:
% predictions of human motion may assign non-zero probability to a wide range of states at a future time, which may severely impede the robot's ability to operate in the shared space with ``absolute safety''
% (only absolute according to the model).
% Therefore, depending on the context, the designers or operators of the system will need to determine what is an acceptable probability that a robot's plan will conflict with the human's future motion.
% Based on this, the robot's online planning algorithm will determine when a motion plan is predicted to be \textit{sufficiently safe}. In our demonstrated system, we use a $1\%$ collision probability threshold for planning. 

% Our goal now is to find efficient robot motion plans that will keep collisions with a human below an acceptable probability.
% Formally, given a current state $x_R^{\text{now}}\in\mathbb{R}^{n_R}$, a cumulative cost ${c:\mathbb{R}^{n_R} \times \mathbb{R}^{m_R} \to \mathbb{R}}$, a probability threshold $P_{\text{th}}\in[0,1]$ and a final time $T$, we define the constrained planning problem:
% \begin{subequations}
% \begin{align}
%         \min_{u_R^{t:T}} &\sum_{\tau=t}^T c(x_R^\tau,u_R^\tau) \label{eq:opt_objective}\\
%         \text{s.t. } & x_R^t = x_R^{\text{now}} \label{eq:opt_initial}\\
%         &x_R^{\tau+1} = \tilde f_R(x_R^\tau,u_R^\tau), \quad \tau\in{t,...,T-1}\label{eq:opt_dynamics}\\
%         & P^{t:T}_\text{coll}:=P\big(\exists \tau\in\{t,...,T\}: \text{coll}(x_R^\tau,x_H^\tau)\big) \le P_{\text{th}}\label{eq:opt_safety}
% \end{align}
% \end{subequations}
% with $\tilde f_R$ a discrete-time approximation of the dynamics~$f_R$. The term $\text{coll}(x_R^t,x_H^t)$ is a Boolean variable indicating whether the human and the robot are in collision.

% The safety analysis necessary to solve this online motion planning problem therefore has two main components, the robot's state and the human's state, both of which are affected by uncertainty in their evolution over time.
% We tackle these two sources of uncertainty through a combined method that draws simultaneously on the two main approaches to uncertain systems: probabilistic and worst-case analysis.

% \example{
% The quadcopter's cost can be a weighted combination of distance traversed and time elapsed on its way to a specified goal: $c(x_R,u_R) = ||u_R||_2 + c_0$.
% }

% The proposed approach in this paper follows two central steps to provide a quantifiable, high-confidence collision avoidance guarantee for the robot's motion around the human. 
% In Section \ref{sec:solution_pred} we present our proposed Bayesian framework for reasoning about the uncertainty inherent in a model's prediction of human behavior. 
% Based on this inference, we demonstrate how to generate a real-time probabilistic prediction of the human's motion over time. 
% Next, in Section \ref{sec:solution_plan} we introduce a theoretical extension to a state-of-the-art, provably safe, real-time robotic motion planner to incorporate our time-varying probabilistic human predictions yielding a quantitative probabilistic safety certificate.

